Statistical Depth Meets Machine Learning: Kernel Mean Embeddings and Depth in Functional Data Analysis

Statistical depth is the act of gauging how representative a point is compared to a reference probability measure. The depth allows introducing rankings and orderings to data living in multivariate, or function spaces. Though widely applied and with much experimental success, little theoretical progress has been made in analysing functional depths. This article highlights how the common $h$-depth and related statistical depths for functional data can be viewed as a kernel mean embedding, a technique used widely in statistical machine learning. This connection facilitates answers to open questions regarding statistical properties of functional depths, as well as it provides a link between the depth and empirical characteristic function based procedures for functional data.

==> Depth.tex <==
We denote by $\calP(\calX)$ the set of Borel probability measures on a general topological space $\calX$. Statistical depth is a method used to assess how standard a given point $x \in \calX$ is compared to a reference distribution $P \in \calP(\calX)$. It has been studied for decades and has its origin in multivariate data analysis, i.e. the case $\calX = \bbR^d$. The first notion of depth was halfspace depth \citep{Tukey1975} which generalizes the quantiles and the median to multivariate data; other well-known depths are simplical depth \cite{Liu1990} or zonoid depth \cite{Koshevoy_Mosler1997, Mosler2002}, the latter extending the expectiles to $\bbR^d$. % Many depths for multivariate data now exist; a comprehensive theory including multiple desiderata for a depth function in $\bbR^d$ can be found in \citep{Liu1999,Zuo2000,Serfling2006}.

The concept of depth for functional data is much more challenging. Standard multivariate depths such as halfspace, simplicial, or zonoid depth are either impossible to be extended to function spaces $\calX$ directly, or degenerate when considered in spaces of high dimension. Also, the desired properties of a depth in $\bbR^d$ do not naturally carry over to spaces of infinite dimension \citep{NietoReyes2016,Gijbels2017}. Nevertheless, also for function spaces $\calX$ multiple notions of depth have been introduced in the last two decades; for a partial overview see \citep{Nagy2016}. These different notions of functional depths have found many applications in data visualisation \cite{Sun_Genton2011}, nonparametric estimation \cite{Fraiman_Muniz2001}, outlier detection \citep{Febrero2008}, classification \citep{LopazPintado2006}, or testing \citep{LopezPintado2009}, to name a few.

The focus of this paper will be $h$-depth \citep{Cuevas2006}, a common functional depth known to be well performing in practice.

\begin{definition}\label{def:h_mode}
Let $\calX$ be a vector space equipped with norm $\norm{\cdot}_{\calX}$, $P\in\calP(\calX)$ and $\kappa\colon[0,\infty)\rightarrow[0,\infty)$ be continuous, non-increasing with $\kappa(0) > 0$ and $\lim_{t\rightarrow\infty}\kappa(t) = 0$. The \emph{$h$-depth} of $x\in\calX$ with respect to $P$ is defined as
\begin{align}
    D_{\kappa}(x;P) = \bbE_{X\sim P}\left[\kappa(\norm{x-X}_{\calX})\right].\label{eq:h_mode}
\end{align}
\end{definition}

\begin{remark}
The $h$ in the name $h$-depth is from the rescaling $\kappa_{h}(\cdot) = h^{-1}\kappa(\cdot/h)$ used in practice with $h>0$. The parameter $h$ plays the role of a bandwidth, but in this context is typically taken to be fixed to a constant rather than altering with new data \citep{Cuevas2007}. For ease of presentation we assume without loss of generality that $h=1$, for other values the proofs are identical with $\kappa_{h}$ replacing $\kappa$. 
\end{remark}

The $h$-depth is a simple and well-performing functional depth, but has been subject only to limited theoretical investigation --- some basic properties of this depth are provided in \citep{Gijbels2017}, and the rates of convergence of its sample version are derived in \cite{Nagy2015}. The $h$-depth has, however, been widely used in practice due to its simple empirical estimate based on a random empirical measure $P_{n} = n^{-1}\sum_{i=1}^{n}\delta_{X_{i}} \in \calP(\calX)$ given by $D_{\kappa}(x;P_{n}) = n^{-1}\sum_{i=1}^{n}\kappa(\norm{x-X_{i}}_{\calX})$. Here, $X_1, \dots, X_n$ is a random sample from $P \in \calP(\calX)$. A common choice of function $\kappa$ in \eqref{eq:h_mode} is $\kappa(t) = e^{-t^{2}/2}$ which is referred to in the literature as \emph{Gauss $h$-depth}.
